MeshCNN: A Network with an Edge

Polygonal meshes provide an efficient representation for 3D shapes. They explicitly capture both shape surface and topology, and leverage non-uniformity to represent large flat regions as well as sharp, intricate features. This non-uniformity and irregularity, however, inhibits mesh analysis efforts using neural networks that combine convolution and pooling operations. In this paper, we utilize the unique properties of the mesh for a direct analysis of 3D shapes using MeshCNN, a convolutional neural network designed specifically for triangular meshes. Analogous to classic CNNs, MeshCNN combines specialized convolution and pooling layers that operate on the mesh edges, by leveraging their intrinsic geodesic connections. Convolutions are applied on edges and the four edges of their incident triangles, and pooling is applied via an edge collapse operation that retains surface topology, thereby, generating new mesh connectivity for the subsequent convolutions. MeshCNN learns which edges to collapse, thus forming a task-driven process where the network exposes and expands the important features while discarding the redundant ones. We demonstrate the effectiveness of our task-driven pooling on various learning tasks applied to 3D meshes.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

SAMPLES = \
	samples/sample-manuscript.tex \
	samples/sample-acmsmall.tex \
	samples/sample-acmlarge.tex \
	samples/sample-acmtog.tex \
	samples/sample-sigconf.tex \
	samples/sample-sigconf-authordraft.tex \
	samples/sample-sigconf-xelatex.tex \
	samples/sample-sigplan.tex \
	samples/sample-sigchi.tex \
	samples/sample-sigchi-a.tex


PDF = $(PACKAGE).pdf ${SAMPLES:%.tex=%.pdf} acmguide.pdf

all:  ${PDF}


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<

samples/%: %
	cp $^ samples

samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex $(notdir $<)
	cd $(dir $@) && pdflatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex $(notdir $<); done

samples/sample-sigconf-xelatex.pdf:  samples/sample-sigconf-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex $(notdir $<)
	cd $(dir $@) && xelatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex $(notdir $<); done

samples/sample-manuscript.pdf \
samples/sample-acmsmall.pdf \
samples/sample-acmlarge.pdf \
samples/sample-acmtog.pdf: samples/samplebody-journals.tex

samples/sample-sigconf.pdf \
samples/sample-sigconf-authordraft.pdf \
samples/sample-sigconf-xelatex.pdf \
samples/sample-sigplan.pdf \
samples/sample-sigchi.pdf: samples/samplebody-conf.tex


.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls


clean:
	$(RM)  $(PACKAGE).cls *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut

distclean: clean
	$(RM) $(PDF) samples/*-converted-to.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all
	zip $@ acmart.pdf acmguide.pdf samples/sample-*.pdf *.cls *.bst


==> figures/configs/cubes.tex <==
\begin{tabular}{c} 
\hline\hline
ResConv $f_{in} \times 32$\\ 
MeshPool $\xrightarrow{} 660$ \\ 
ResConv $32 \times 64$ \\ 
MeshPool $\xrightarrow{} 510$ \\ 
ResConv $64 \times 128$ \\ 
MeshPool $\xrightarrow{} 360$ \\ 
ResConv $128 \times 128$ \\ 
MeshPool $\xrightarrow{} 210$ \\ 
ResConv $128 \times 128$ \\ 
MeshPool $\xrightarrow{} 195$ \\ 
FC $ (195 \cdot 128) \times 100 $ \\ 
FC $ 100 \times 23 $ \\ 
\hline\hline
Cubes
\end{tabular}

==> figures/coseg/figure.tex <==
\begin{figure}
\newcommand{\cfig}{2.7}
\begin{tabular}{ccc}
\includegraphics[width=\cfig cm]{figures/coseg/0014.jpg} &
\includegraphics[width=\cfig cm]{figures/coseg/0081.jpg} &
\includegraphics[width=\cfig cm]{figures/coseg/0103.jpg} \\
\includegraphics[width=\cfig cm]{figures/coseg/0152.jpg} &
\includegraphics[width=\cfig cm]{figures/coseg/0191.jpg} &
\includegraphics[width=\cfig cm]{figures/coseg/0259.jpg} \\

%\adjincludegraphics[width=\cfig cm,trim={{0.25\width} {0.12\height} {0.25\width} {0.12\height}},clip]{figures/coseg/0081.jpg} &
%\adjincludegraphics[width=\cfig cm,trim={{0.25\width} {0.12\height} {0.25\width} %{0.12\height}},clip]{figures/coseg/0103.jpg} &
%\adjincludegraphics[width=\cfig cm,trim={{0.25\width} {0.12\height} {0.25\width} %{0.12\height}},clip]{figures/coseg/0152.jpg} &
%\adjincludegraphics[width=\cfig cm,trim={{0.25\width} {0.12\height} {0.25\width} %{0.12\height}},clip]{figures/coseg/0191.jpg} &
%\adjincludegraphics[width=\cfig cm,trim={{0.25\width} {0.12\height} {0.25\width} %{0.12\height}},clip]{figures/coseg/0259.jpg} \\

\end{tabular}
\caption{Semantic segmentation results on (held out) test shapes. \ourmethod{} uses mesh pooling to learn to collapse edges from the same segments, which are unrolled back to the original input mesh resolution via the mesh unroll layer.}
\label{fig:coseg}
\end{figure}


%
\begin{comment}
\begin{table}
\begin{center}
\begin{tabular}{||c c c c c||} 
\hline
\multicolumn{4}{c}{COSEG}\\
\hline
Method & capacity & Vases & Chairs & Telealiens \\ [0.2ex] 
\hline\hline\hline\hline\hline
MeshCNN & $0.019 M$ & $89.1\%$ & $73.7\%$ & $75.8\%$ \\ 
\hline\hline\hline\hline
PointNet & $1.670 M$ & $91.5\%$ & $70.2\%$ &  $54.4\%$\\ 
PointNet++ &  M & $\%$ & $\%$ &  $\%$\\ 
%PointCNN & $3.88 M$ & $\%$ & $\%$ &  $\%$\\ 
\end{tabular}
\end{center}
\caption{Test results on COSEG benchmark.}
\end{table}
\label{tab:cosegtbl}
\end{comment}

==> figures/cubes/figure_pc.tex <==
\begin{figure}
\includegraphics[width=7cm]{figures/cubes/cube_pt-01.png}
\caption{An example of two different classes (\emph{apple} and \emph{heart}) in the mesh and pointcloud form. While it is immediately obvious which mesh belongs to the \emph{heart} or \emph{apple} class, the two pointcloud samples appear indistinguishable.}
\label{fig:pt_cubes}
\end{figure}

==> figures/dfaust/figure.tex <==
\begin{figure}
\includegraphics[width=18cm]{figures/overview_pooling/neighbors3-01.png}
\caption{\dc{(a) Features are computed for the edges by applying convolutions with the four edges of the two incident triangles. The four blue edges are incident to the edge in red. (b) and (c) demonstrate a pooling step. In (b) the red edge in (a) is collapsing to a point, and the four incident (blue) lines collapse into the two (blue) edges in (c). Note that an edge collapse five edges are converted into two edges.}}
\label{fig:coco}
\end{figure}

==> figures/dfaust/swaps/figure.tex <==
\begin{figure}
\newcommand{\vfig}{8.3}
\begin{tabular}{c}
%<left> <lower> <right> <upper>
\adjincludegraphics[width=\vfig cm,trim={{.01\width} {.12\height} {.05\width} {.18\height}},clip]{figures/dfaust/swaps/same_face_zoom-03.png} \\
\adjincludegraphics[width=\vfig cm,trim={{.01\width} {.09\height} {.01\width} {.17\height}},clip]{figures/dfaust/swaps/same_body_zoom-02.png} \\

\end{tabular}
\caption{DFAUST head swap classification examples. Top: the same head on different bodies. Bottom: same body with different heads.}
\label{fig:dfaustswap}
\end{figure}



==> figures/dfaust/swaps/table.tex <==
\begin{table}
\begin{center}
\begin{tabular}{||c c c c||} 
\hline
\multicolumn{4}{c}{\rh{DFAUST Head Swap}}\\
\hline
Method & Input Resolution & Face & Body \\ [0.2ex] 
\hline\hline\hline\hline\hline
MeshCNN & 1100 & $ \textbf{99.75} \%$ & $ \%$ \\ 
% other approaches
\hline\hline\hline\hline
%PointNet & non-uniform & $ 21.98 \%$ & $ 59.44 \%$ \\ 
PointNet & 2500 & $ \%$ & $ \%$ \\ 
%PointNet++ &  non-uniform & $ 56.35 \%$ & $ 96.98\%$ \\ 
\hline
\end{tabular}
\end{center}
\caption{\rh{Test accuracy on head swap benchmark.}}
\label{tab:dfaustswap}
\end{table}


==> figures/eval/xyzpoints/strech_res.tex <==
\begin{figure}
\setlength{\tabcolsep}{1pt}
\includegraphics[width=2cm]{figures/eval/xyzpoints/stretch_chairs2.png} \\
\begin{tabular}{cc|cc}
%<left> <lower> <right> <upper>
%
%\hline
%
\adjincludegraphics[width=1.3 cm,trim={{0.45\width} {0.0\height} {0.3\width} {0.0\height}},clip]{figures/eval/xyzpoints/0245_0_xyz.png} &
%
\adjincludegraphics[width=1.3 cm,trim={{0.45\width} {0.0\height} {0.3\width} {0.0\height}},clip]{figures/eval/xyzpoints/0245_0.png} &
%
\adjincludegraphics[width=1.3 cm,trim={{0.45\width} {0.0\height} {0.3\width} {0.0\height}},clip]{figures/eval/xyzpoints/0315_0_xyz.png} &
\adjincludegraphics[width=1.3 cm,trim={{0.45\width} {0.0\height} {0.3\width} {0.0\height}},clip]{figures/eval/xyzpoints/0315_0.png} \\
%3D points & geometric \\
\end{tabular}
%\includegraphics[width=2cm]{figures/eval/xyzpoints/0245_0.png} \\
%\includegraphics[width=2cm]{figures/eval/xyzpoints/0245_0_xyz.png} &
\caption{\rh{Robustness of Differential Features. We evaluate generalization on stretched set (top). Using \ourmethod{} geometric features compared to standard $3$D points (edge midpoints). While both achieve high accuracy on the standard test set, using \ourmethod{} features generalizes well to the stretched set.}}
\label{fig:strech_chair_set}
\end{figure}
%\adjincludegraphics[width=2 cm,trim={{0.0\width} {0.08\height} {0.28\width} {0.08\height}},clip]{figures/eval/xyzpoints/0245_0.png} \\

==> figures/meshes/figure_arch.tex <==
\begin{figure}
\includegraphics[width=7cm]{figures/meshes/arch_simple-01.png}
\caption{Illustration of how \ourmethod{} combines the convolution and pooling operations. The edge neighbors ($\mathcal{N}$) are extracted from the mesh ($\mathcal{M}$), which are dynamically updated at each pooling layer $l$.}
\label{fig:arch}
\end{figure}

==> figures/meshes/figure_overview.tex <==
\begin{figure}
\includegraphics[width=6cm]{figures/meshes/components-01.png}
\caption{Each of the building blocks implemented in \ourmethod{}. \emph{features:} takes a list of edges and converts them into a $6$-dimensional feature (the dihedral angle, two inner angles, two edge-length ratios for each face and one global edge length ratio. \emph{conv:} takes a list of features and $N$ (a matrix of indices describing the edge neighbors) used to define the convolution. \emph{pool:} takes the edge features and reduces them by simplification and updating the neighbors. \emph{unroll:} history for where each collapsed edge came from in the original list.}
\label{fig:blocks}
\end{figure}

==> figures/overview.tex <==
\section{Overview: Applying CNN on Meshes}
\label{sec:overview}

Polygonal meshes are the most fundamental and commonly used 3D data representation in computer graphics. The non-uniform mesh representation is adaptable to the underlying geometry; large flat regions use a small number of large polygons, while detailed regions use a larger number of polygons (see Figure \ref{fig:adaptivemesh}). \rh{Furthermore, a mesh explicitly represents the topology of a surface: faithfully describing intricate structures while disambiguating proximity from nearby surfaces (see Figure \ref{fig:euc_geod}). The effective mesh representation inherently captures sharp features (common in man-made 3D objects), as opposed to  point set representations that struggle under these conditions.}

\input{figures/teaser/figure_nbrs.tex}


Realizing our goal to apply the CNN paradigm directly onto triangular meshes, necessitates an analogous definition and implementation of the standard operators that are the backbone of every CNN. Image-based CNNs contain convolutional, non-linearity and simplification (pooling) layers within their pipeline, a combination which results in a robust learning framework. As opposed to images which are represented on a regular grid of discrete values, the key challenge in mesh analysis is its inherent irregularity and non-uniformity. 

\shflc{This paragraph belongs to the intro or conclusion, or simply delete it In our work, we aim to exploit these challenging and unique properties, rather than bypassing them. Accordingly, we design our network to deliberately apply convolution and pooling operations directly on the constructs of the mesh, and avoid conversion to a regular and uniform representation. While image-based CNNs are often restricted to predetermined input dimensions, a notable advantage of the nature of our simplification, which is a mesh-based simplification using edge collapse, is that it provides flexibility with regards to the output dimensions of the pooling layer. In other words, an arbitrarily sized mesh is input to the network and simplified by the pooling layers in a dynamic manner, such that the desired resolution is reached before proceeding to the final fully connected layers. As this resolution highly influences the capacity and computational complexity of the network, it should be adjusted appropriately.}

\input{figures/meshes/figure.tex}

\begin{wrapfigure}{R}{0.1\textwidth}
\begin{center}
\includegraphics[width=0.1\textwidth]{figures/meshes/features.png}
\end{center}
\end{wrapfigure}

In \ourmethod{}, the edges of a mesh are analogous to pixels in an image, since they are the basic building blocks for all CNN operations.
Just as images start with a basic input feature: an $RGB$ value per pixel; \ourmethod{} starts with a basic geometric feature per edge.
The input edge feature is a $5$-dimensional vector for every edge: the dihedral angle, two inner angles and two edge-length ratios for each face. The edge ratio is between the length of the edge and the the perpendicular (dotted) line for each adjacent face. \shflc{is it really 5, or do you add (x,y,z)?}
Observe that these features are all \textit{relative}, making them invariant to \textit{translation}, \textit{rotation} and \textit{uniform scale}.
%\dc{The inset figure is not in the correct paragraph, should be here...}
%As with image CNNs, the input (edge) feature values lose their meaning after passing through the first convolution. 

Our network operates and learns features on the edges of the mesh, as they form a consistent and stable set of entities, despite the overall irregular nature of the mesh. Each edge is adjacent to two triangles (faces), defining a natural, fixed-sized neighborhood of edges, illustrated in Figure \ref{fig:coco}(a), where the red edge has four one-ring edges shown in blue. Such an edge neighborhood forms a regular sized receptive field \rh{to apply the learned \textbf{convolution} filters.}

The \textbf{pooling} operation is accomplished by an edge collapse process, as \rh{illustrated} in Figure \ref{fig:coco} (b) and (c). In (b), the dashed edge is collapsing to a point, and, subsequently, the four incident edges (blue) merge into the two (blue) edges in (c). Note that in this edge collapse operation, five edges are transformed into two. 
The operator is prioritized by the \rh{(smallest norm) edge features}, thereby allowing the network to select which parts of the mesh to simplify, and which to leave intact. This creates a task-aware process, where the network learns to determine object part importance with respect to its mission (see Figure \ref{fig:task_driven_pool}).





%Polygonal meshes are the most fundamental and commonly used 3D data representation in computer graphics. A mesh explicitly represents both the geometry and topology of a surface. It provides direct access to geodesic neighborhood information, faithfully describing intricate surface structures while disambiguating Euclidean proximity from on-surface, geodesic proximity (see Figure \ref{fig:euc_geod}). Furthermore, the mesh administers a non-uniform representation that is adaptable to the underlying shape geometry. Large flat regions can be represented by a small number of large polygons, with a larger number of flexibly sized polygons covering detailed, non-smooth regions (see Figure \ref{fig:adaptivemesh}). The agility of the mesh reflects directly upon its effectiveness as a representation, and is apparent by simply considering its inherent ability to capture sharp shape features common in man-made 3D objects, as opposed to point set representations that struggle under these conditions. 


==> figures/pooling/figure.tex <==
\begin{figure*}
%\includegraphics[width=6cm]{figures/figure2-_alvar_alto_armchair.png} 
%\begin{tabular}{c c c}
%\includegraphics[width=2cm]{figures/under-construction.png} &
%\includegraphics[width=2cm]{figures/under-construction.png} &
%\includegraphics[width=2cm]{figures/under-construction.png} \\
%\end{tabular}
%\centering
\newcommand{\vfig}{2}
\setlength\tabcolsep{10pt}
\renewcommand{\arraystretch}{2.5}
\begin{tabular}{c c c c c c}
\adjincludegraphics[width=\vfig cm,trim={{.35\width} {.15\height} {.35\width} {.14\height}},clip]{figures/teaser/pooling/029500.png} &
\adjincludegraphics[width=\vfig cm,trim={{.35\width} {.15\height} {.35\width} {.14\height}},clip]{figures/teaser/pooling/0295_pool0_h01.png} &
\adjincludegraphics[width=\vfig cm,trim={{.35\width} {.15\height} {.35\width} {.14\height}},clip]{figures/teaser/pooling/0295_pool1_h02.png} &
\adjincludegraphics[width=\vfig cm,trim={{.35\width} {.15\height} {.35\width} {.14\height}},clip]{figures/teaser/pooling/0295_pool2_h03.png} &
\adjincludegraphics[width=\vfig cm,trim={{.35\width} {.15\height} {.35\width} {.14\height}},clip]{figures/teaser/pooling/0295_pool3_h04.png} &
\adjincludegraphics[width=\vfig cm,trim={{.35\width} {.15\height} {.35\width} {.14\height}},clip]{figures/teaser/pooling/0295_poolh_405.png} \\
%
\adjincludegraphics[width=\vfig cm,trim={{.35\width} {.15\height} {.35\width} {.14\height}},clip]{figures/teaser/pooling/029500.png} &
\adjincludegraphics[width=\vfig cm,trim={{.35\width} {.15\height} {.35\width} {.14\height}},clip]{figures/teaser/pooling/0295_poolt_006.png} &
\adjincludegraphics[width=\vfig cm,trim={{.35\width} {.15\height} {.35\width} {.14\height}},clip]{figures/teaser/pooling/0295_poolt_107.png} &
\adjincludegraphics[width=\vfig cm,trim={{.35\width} {.15\height} {.35\width} {.14\height}},clip]{figures/teaser/pooling/0295_poolt_208.png} &
\adjincludegraphics[width=\vfig cm,trim={{.35\width} {.15\height} {.35\width} {.14\height}},clip]{figures/teaser/pooling/0295_poolt_309.png} &
\adjincludegraphics[width=\vfig cm,trim={{.35\width} {.15\height} {.35\width} {.14\height}},clip]{figures/teaser/pooling/0295_poolt_410.png} \\
\end{tabular}
%\includegraphics[width=6cm]{figures/under-construction.png}
\caption{\rh{Pooling on learned edge features allows MeshCNN to determine which parts of the mesh to simplify. Different than a geometric simplification (which computes the geometric distortion of removing each edge), MeshCNN learns which edge to collapse based on the task. The top row is the intermediate simplification results on training a network to classify whether vases have a handle or not vs. the bottom row  which is the result of training a network to classify whether a vase has a neck (top piece) or not.} \rg{RG: I suggest changing the order such that the handle cases will be in the top two rows and neck cases in the bottom two rows. In this way, we will be able to say in this caption "The top two rows are the ... vs. the bottom two rows which are...". I think it will make the caption clearer.}}
\label{fig:teaser}
\end{figure*}


%

==> figures/pooling/figure_shadows.tex <==
\begin{figure}
\newcommand{\vfig}{8}
\begin{tabular}{c}
%<left> <lower> <right> <upper>
\adjincludegraphics[width=\vfig cm,trim={{0.0\width} {0.0\height} {0.0\width} {0.0\height}},clip]{figures/pooling/vase_pooling_tight-03.png} \\
\end{tabular}
\caption{Pooling on learned edge features allows \ourmethod{} to determine which parts of the mesh to simplify. Unlike a geometric simplification (which computes the geometric distortion of removing each edge), \ourmethod{} learns which edge to collapse based on the task. The top row is the intermediate simplification results on training a network to classify whether vases have a handle or not vs. the bottom row, which is the result of training a network to classify whether a vase has a neck (top piece) or not.}
\label{fig:task_driven_pool}
\end{figure}




==> figures/teaser/figure.tex <==
\begin{figure}[t!]
\newcommand{\vfig}{8.3}
\begin{center}
\begin{tabular}{c}
\adjincludegraphics[width=\vfig cm,trim={{0.1\width} {.13\height} {.12\width} {.5\height}},clip]{figures/teaser/teaser_v5b.png} \\
%result \qquad  \: 
%pool $1$ \qquad \: \:
%pool $2$ \qquad \:  
%pool $3$ \qquad \\
\end{tabular}
\end{center}
\caption{\ourmethod{} predicts a semantic segmentation class per edge (\textit{result} on the left). The input mesh passes through a neural network containing a series of mesh convolutions and mesh pooling layers, which are optimized for the segmentation task. We reduce the feature map size via an edge collapse operation, which is highly irregular and adapts to the task. Notice how the intermediate pooled meshes (shown after mesh pool layer $1$, $2$ and $3$) have reduced the entire vase handle into a single edge.} \rg{RG: I suggest adding here subtitles like in Fig. 11. I think it will make the figure clearer.}
\label{fig:teaser}
\end{figure}

\begin{comment}

\begin{figure}[b!]
\begin{tabular}{c}
\newcommand{\vfig}{8}
%\multicolumn{4}{c}{}\\
\adjincludegraphics[width=\vfig cm,trim={{0.01\width} {.05\height} {.01\width} {.38\height}},clip]{figures/teaser/teaser_v2.png} \\
result & pool $1$ & pool $2$ & pool $3$ \\
\end{tabular}
\caption{\rh{\ourmethod{} predicts a semantic segmentation class per edge: \textit{result}. The input mesh passes through a neural network containing mesh convolutions and $3$ mesh pooling layers, which are The intermediate pooled meshes are}}
\label{fig:teaser}
\end{figure}



\begin{figure}[b!]
\newcommand{\vfig}{8}
\begin{center}
\begin{tabular}{c c c c}
\multicolumn{4}{c}{\adjincludegraphics[width=\vfig cm,trim={{0.01\width} {.05\height} {.01\width} {.38\height}},clip]{figures/teaser/teaser_v4.png}}\\
result & pool $1$ & pool $2$ & pool $3$ \\
\end{tabular}
\end{center}
\caption{\rh{\ourmethod{} predicts a semantic segmentation class per edge: \textit{result}. The input mesh passes through a neural network containing mesh convolutions and $3$ mesh pooling layers, which are The intermediate pooled meshes are}}
\label{fig:teaser}
\end{figure}





\end{comment}
